Fairway: A Way to Build Fair ML Software

Machine learning software is increasingly being used to make decisions that affect people's lives. But sometimes, the core part of this software (the learned model), behaves in a biased manner that gives undue advantages to a specific group of people (where those groups are determined by sex, race, etc.). This "algorithmic discrimination" in the AI software systems has become a matter of serious concern in the machine learning and software engineering community. There have been works done to find "algorithmic bias" or "ethical bias" in the software system. Once the bias is detected in the AI software system, the mitigation of bias is extremely important. In this work, we a)explain how ground-truth bias in training data affects machine learning model fairness and how to find that bias in AI software,b)propose a methodFairwaywhich combines pre-processing and in-processing approach to remove ethical bias from training data and trained model. Our results show that we can find bias and mitigate bias in a learned model, without much damaging the predictive performance of that model. We propose that (1) test-ing for bias and (2) bias mitigation should be a routine part of the machine learning software development life cycle. Fairway offers much support for these two purposes.

==> options.tex <==
\begin{table}

%\captionsetup{font=footnotesize}
\caption{Hyperparameter  options
seen in recent SE papers~\cite{ghotra2015revisiting,fu2016tuning,agrawal2018better,agrawal2018wrong} and in  the documentation of a widely-used data mining library
(Scikit-learn~\cite{pedregosa2011scikit}) for a list of options not explored
in those studies.
While this list is incomplete, it does include many
of the   hyperparameter optimizations being explored in the literature. }\label{tbl:options}
\footnotesize
 
\begin{tabular}{|p{.95\linewidth}|}\hline
\textbf{Learners:}  


\noindent
\bi
\item DecisionTreeClassifier(criterion=b, splitter=c, min\_samples\_split=a)
    \bi
   \item a, b, c= randuniform(0.0,1.0), randchoice([`gini',`entropy']), \newline randchoice([`best',`random'])
   \ei
\item RandomForestClassifier(n\_estimators=a,criterion=b,  min\_samples\_split=c)
    \bi
   \item a,b,c = randint(50, 150), randchoice(['gini', 'entropy']),\newline randuniform(0.0, 1.0) 
   \ei
\item LogisticRegression(penalty=a, tol=b, C=float(c))
    \bi
    \item a,b,c=randchoice([`l1',`l2']), randuniform(0.0,0.1), randint(1,500)
    \ei 
\item MultinomialNB(alpha=a) = randuniform(0.0,0.1)
\item KNeighborsClassifier(n\_neighbors=a, weights=b, p=d, metric=c)
    \bi
    \item a, b,c  = randint(2, 25), randchoice([`uniform', `distance']), \newline randchoice([`minkowski',`chebyshev'])
    \item if c=='minkowski': d= randint(1,15)  else:  d=2
    \ei
     
    
\ei
\\\hline

{\bf Pre-processors for   defect prediction, Issue lifetime, Bad   Smells:} 

\bi 
\item StandardScaler
\item MinMaxScaler
\item MaxAbsScaler
\item RobustScaler(quantile\_range=(a, b)) =  randint(0,50), randint(51,100) 
\item KernelCenterer
\item QuantileTransformer(n\_quantiles=a,  output\_distribution=c, subsample=b)
    \bi
    \item a, b = randint(100, 1000), randint(1000, 1e5)
    \item c = randchoice([`normal',`uniform'])
    \ei
\item Normalizer(norm=a) = randchoice([`l1', `l2',`max'])
  
\item Binarizer(threshold=a) =  randuniform(0,100)
   
    \item SMOTE(a=n\_neighbors, b=n\_synthetics,  c=Minkowski\_exponent)
    \bi
    \item a,b = randit(1,20),randchoice(50,100,200,400)
    \item c = randuniform(0.1,5)
    \ei
\ei

 \\\hline
{\bf Pre-Processors for Text mining:}  
 
\bi
\item CountVectorizer(max\_df=a, min\_df=b) = randint(100, 1000), randint(1, 10)
\item TfidfVectorizer(max\_df=a, min\_df=b, norm=c)
    \bi
    \item a, b,c = randint(100, 1000), randint(1, 10), randchoice([`l1', `l2', None])
    \ei
\item HashingVectorizer(n\_features=a, norm=b)
    \bi
    \item a = randchoice([1000, 2000, 4000, 6000, 8000, 10000])
    \item b = randchoice([`l1', `l2', None])
    \ei
\item LatentDirichletAllocation(n\_components=a, doc\_topic\_prior=b,\newline topic\_word\_prior=c,
                                   learning\_decay=d,
                                   learning\_offset=e,batch\_size=f)
    \bi
    \item a, b, c = randint(10, 50), randuniform(0, 1),  randuniform(0, 1)
    \item d, e  = randuniform(0.51, 1.0), randuniform(1, 50), 
    \item f = randchoice([150,180,210,250,300])
    \ei
\ei 


 \\\hline
 \end{tabular}

\end{table}
